Forecasting the cost of drought events in France by Super Learning

Drought events are the second most expensive type of natural disaster within the French legal framework known as the natural disasters compensation scheme. In recent years, drought events have been remarkable in their geographical scale and intensity. We develop and apply a new methodology to forecast the cost of a drought event in France. The methodology hinges on Super Learning (van der Laan et al., 2007; Benkeser et al., 2018), a general aggregation strategy to learn a feature of the law of the data identified through an ad hoc risk function by relying on a library of algorithms. The algorithms either compete (discrete Super Learning) or collaborate (continuous Super Learning), with a cross-validation scheme determining the best performing algorithm or combination of algorithms, respectively. Our Super Learner takes into account the complex dependence structure induced in the data by the spatial and temporal nature of drought events.

==> copernicus.tex <==
\newif\ifprp             \DeclareOption{prp}     {\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue                  \@bartrue \prptrue}
\newif\ifgtes            \DeclareOption{gtes}    {\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue                  \@bartrue \gtestrue}
\newif\ifcopyediting     \DeclareOption{copyediting}{\copyeditingtrue\@noreftrue}
\newif\ifsmsps           \DeclareOption{smsps}   {                  \smspstrue}
\newif\ifegusphere  \DeclareOption{egusphere}{\@twostagejnltrue\eguspheretrue}
            \DeclareOption{egusphered}{\@stage@finalfalse\eguspheretrue}
\newif\ifsand  \DeclareOption{sand}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sandtrue}
\newif\ifpolf  \DeclareOption{polf}{\@sansseriffacetrue\@sansserifheadertrue\@bartrue\polftrue}
\newif\ifjbji  \DeclareOption{jbji}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\jbjitrue}
\newif\ifmr  \DeclareOption{mr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\mrtrue}
            \DeclareOption{mrd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\mrtrue}
\newif\ifejm  \DeclareOption{ejm}{\@abstractcenteredtrue\@bartrue\ejmtrue}
\newif\ifwcd  \DeclareOption{wcd}{\@twostagejnltrue\wcdtrue}
            \DeclareOption{wcdd}{\@stage@finalfalse\wcdtrue}
\newif\ifgchron  \DeclareOption{gchron}{\@sansseriffacetrue\@sansserifheadertrue\@twostagejnltrue\gchrontrue}
            \DeclareOption{gchrond}{\@sansseriffacetrue\@sansserifheadertrue\@stage@finalfalse\gchrontrue}
\newif\ifdeuquasp  \DeclareOption{deuquasp}{\@sansseriffacetrue\@sansserifheadertrue\@abstractindentedtrue\@bartrue\@seclinetrue\deuquasptrue}
\newif\ifgc  \DeclareOption{gc}{\@sansseriffacetrue\@sansserifheadertrue\@bartrue\@twostagejnltrue\gctrue}
            \DeclareOption{gcd}{\@sansseriffacetrue\@sansserifheadertrue\@bartrue\@stage@finalfalse\gctrue}
\newif\ifegqsj  \DeclareOption{egqsj}{\@sansseriffacetrue\@sansserifheadertrue\@abstractindentedtrue\@bartrue\@seclinetrue\egqsjtrue}
\newif\ifjm  \DeclareOption{jm}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\jmtrue}
\newif\ifwes  \DeclareOption{wes}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\westrue}
            \DeclareOption{wesd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\westrue}
\newif\ifaab  \DeclareOption{aab}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\aabtrue}
\newif\ifpiahs  \DeclareOption{piahs}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\piahstrue}
\newif\ifascmo  \DeclareOption{ascmo}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@corrigendumtrue\@editorialnotetwoctrue\ascmotrue}
\newif\ifpb  \DeclareOption{pb}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\pbtrue}
\newif\ifsoil  \DeclareOption{soil}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\soiltrue}
            \DeclareOption{soild}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\soiltrue}
\newif\ifangeocom  \DeclareOption{angeocom}{\@bartrue\@twostagejnltrue\angeocomtrue}
            \DeclareOption{angeocomd}{\@bartrue\@stage@finalfalse\angeocomtrue}
\newif\ifwe  \DeclareOption{we}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\wetrue}
\newif\ifsdpd  \DeclareOption{sdpd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdpdtrue}
\newif\ifsdwr  \DeclareOption{sdwr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdwrtrue}
\newif\ifsdtd  \DeclareOption{sdtd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdtdtrue}
\newif\ifsdpr  \DeclareOption{sdpr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdprtrue}
\newif\ifsdsr  \DeclareOption{sdsr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdsrtrue}
\newif\ifasr  \DeclareOption{asr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\asrtrue}
\newif\ifms  \DeclareOption{ms}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\mstrue}
\newif\ifjsss  \DeclareOption{jsss}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\jssstrue}
\newif\ifhgss  \DeclareOption{hgss}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\hgsstrue}
            \DeclareOption{hgssd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\hgsstrue}
\newif\ifgh  \DeclareOption{gh}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\ghtrue}
\newif\ifesurf  \DeclareOption{esurf}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\esurftrue}
            \DeclareOption{esurfd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\esurftrue}
\newif\ifessd  \DeclareOption{essd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@twostagejnltrue\essdtrue}
            \DeclareOption{essdd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@stage@finalfalse\essdtrue}
\newif\ifdwes  \DeclareOption{dwes}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@twostagejnltrue\dwestrue}
            \DeclareOption{dwesd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@stage@finalfalse\dwestrue}
\newif\iftc  \DeclareOption{tc}{\@twostagejnltrue\tctrue}
            \DeclareOption{tcd}{\@stage@finalfalse\tctrue}
\newif\ifse  \DeclareOption{se}{\@bartrue\@twostagejnltrue\setrue}
            \DeclareOption{sed}{\@bartrue\@stage@finalfalse\setrue}
\newif\ifos  \DeclareOption{os}{\@twostagejnltrue\ostrue}
            \DeclareOption{osd}{\@stage@finalfalse\ostrue}
\newif\ifnpg  \DeclareOption{npg}{\@editorialnotedtrue\@twostagejnltrue\npgtrue}
            \DeclareOption{npgd}{\@stage@finalfalse\npgtrue}
\newif\ifnhess  \DeclareOption{nhess}{\@editorialnotedtrue\@twostagejnltrue\nhesstrue}
            \DeclareOption{nhessd}{\@stage@finalfalse\nhesstrue}
\newif\ifhess  \DeclareOption{hess}{\@twostagejnltrue\hesstrue}
            \DeclareOption{hessd}{\@stage@finalfalse\hesstrue}
\newif\ifgmd  \DeclareOption{gmd}{\@twostagejnltrue\gmdtrue}
            \DeclareOption{gmdd}{\@stage@finalfalse\gmdtrue}
\newif\ifgi  \DeclareOption{gi}{\@corrigendumtrue\@editorialnotetwoctrue\@editorialnotedtrue\@twostagejnltrue\gitrue}
            \DeclareOption{gid}{\@stage@finalfalse\gitrue}
\newif\ifesd  \DeclareOption{esd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\esdtrue}
            \DeclareOption{esdd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\esdtrue}
\newif\ifcp  \DeclareOption{cp}{\@sansseriffacetrue\@sansserifheadertrue\@twostagejnltrue\cptrue}
            \DeclareOption{cpd}{\@sansseriffacetrue\@sansserifheadertrue\@stage@finalfalse\cptrue}
\newif\ifastra  \DeclareOption{astra}{\astratrue}
\newif\ifars  \DeclareOption{ars}{\arstrue}
\newif\ifangeo  \DeclareOption{angeo}{\@twostagejnltrue\angeotrue}
            \DeclareOption{angeod}{\@stage@finalfalse\angeotrue}
\newif\ifamt  \DeclareOption{amt}{\@twostagejnltrue\amttrue}
            \DeclareOption{amtd}{\@stage@finalfalse\amttrue}
\newif\ifadgeo  \DeclareOption{adgeo}{\adgeotrue}
\newif\iffr  \DeclareOption{fr}{\frtrue}
\newif\ifbg  \DeclareOption{bg}{\@firstbartrue\@twostagejnltrue\bgtrue}
            \DeclareOption{bgd}{\@firstbartrue\@stage@finalfalse\bgtrue}
\newif\ifacp  \DeclareOption{acp}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@twostagejnltrue\acptrue}
            \DeclareOption{acpd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@stage@finalfalse\acptrue}



\def\@addjournalconfig{%


\ifcopyediting% Definition of layout used for copy-editing track changes document
  \def\@journalurl{}
  \def\@sentence{\textcolor[rgb]{1,0.58,0.25}{%
    Copy-Editing track changes document -- Do not use for proof-reading}}
  \let\@journalnameabbreviation\@sentence
  \if@sansserifface
    \definecolor{textcol}{rgb}{0,0,0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{gray}{0.8}
    \definecolor{rulecol}{gray}{0.8}
  \fi
\fi

\ifacp%classical
  \def\@journalname{Atmospheric Chemistry and Physics}
  \def\@journalnameabbreviation{Atmos. Chem. Phys.}
  \def\@journalnameshort{ACP}
  \def\@journalnameshortlower{acp}
  \def\@journalstartyear{2001}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.atmos-chem-phys.net}
    \def\@journallogo{\includegraphics{ACP_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.447,0.737}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.447,0.737}
  \else
    \def\@journalurl{www.atmos-chem-phys-discuss.net}
    \def\@journallogo{\includegraphics{ACPD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Atmospheric Chemistry\\ and Physics (ACP). Please refer to the corresponding final paper in ACP if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.58,0.91}
      \definecolor{buttonbackground}{rgb}{0.0,0.58,0.91}
      \definecolor{paneltext}{rgb}{0.0,0.58,0.91}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifbg%classical
  \def\@journalname{Biogeosciences}
  \def\@journalnameabbreviation{Biogeosciences}
  \def\@journalnameshort{BG}
  \def\@journalnameshortlower{bg}
  \def\@journalstartyear{2004}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.biogeosciences.net}
    \def\@journallogo{\includegraphics{BG_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.0,0.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.612,0.698,0.145}
  \else
    \def\@journalurl{www.biogeosciences-discuss.net}
    \def\@journallogo{\includegraphics{BGD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Biogeosciences (BG).\\ Please refer to the corresponding final paper in BG if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.612,0.698,0.145}
      \definecolor{buttonbackground}{rgb}{0.612,0.698,0.145}
      \definecolor{paneltext}{rgb}{0.612,0.698,0.145}
      \definecolor{buttontext}{rgb}{0.612,0.0,0.055}
    \fi
  \fi
\fi
\iffr%classical
  \def\@journalname{Fossil Record}
  \def\@journalnameabbreviation{Foss. Rec.}
  \def\@journalnameshort{FR}
  \def\@journalnameshortlower{fr}
  \def\@journalstartyear{1998}
  \def\@sentence{Published by Copernicus Publications on behalf of the Museum f{\"u}r Naturkunde Berlin.}
  \def\@journalurl{www.foss-rec.net}
  \def\@journallogo{\includegraphics{FR_Logo.pdf}}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifadgeo%classical
  \def\@journalname{Advances in Geosciences}
  \def\@journalnameabbreviation{Adv. Geosci.}
  \def\@journalnameshort{ADGEO}
  \def\@journalnameshortlower{adgeo}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \def\@journalurl{www.adv-geosci.net}
  \def\@journallogo{\includegraphics{ADGEO_Logo.pdf}}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifamt%classical
  \def\@journalname{Atmospheric Measurement Techniques}
  \def\@journalnameabbreviation{Atmos. Meas. Tech.}
  \def\@journalnameshort{AMT}
  \def\@journalnameshortlower{amt}
  \def\@journalstartyear{2008}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.atmos-meas-tech.net}
    \def\@journallogo{\includegraphics{AMT_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.atmos-meas-tech-discuss.net}
    \def\@journallogo{\includegraphics{AMTD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Atmospheric Measurement\\ Techniques (AMT). Please refer to the corresponding final paper in AMT if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.259,0.475}
      \definecolor{buttonbackground}{rgb}{0.0,0.259,0.475}
      \definecolor{paneltext}{rgb}{0.0,0.259,0.475}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifangeo%classical
  \def\@journalname{Annales Geophysicae}
  \def\@journalnameabbreviation{Ann. Geophys.}
  \def\@journalnameshort{ANGEO}
  \def\@journalnameshortlower{angeo}
  \def\@journalstartyear{1983}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.ann-geophys.net}
    \def\@journallogo{\includegraphics{ANGEO_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifars%classical
  \def\@journalname{Advances in Radio Sciences}
  \def\@journalnameabbreviation{Adv. Radio Sci.}
  \def\@journalnameshort{ARS}
  \def\@journalnameshortlower{ars}
  \def\@journalstartyear{2003}
  \def\@sentence{Published by Copernicus Publications on behalf of the URSI Landesausschuss in der Bundesrepublik Deutschland e.V.}
  \def\@journalurl{www.adv-radio-sci.net}
  \def\@journallogo{\includegraphics{ARS_Logo.pdf}}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifastra%classical
  \def\@journalname{Astrophysics and Space Sciences Transactions}
  \def\@journalnameabbreviation{Astrophys. Space Sci. Trans.}
  \def\@journalnameshort{ASTRA}
  \def\@journalnameshortlower{astra}
  \def\@journalstartyear{2004}
  \def\@sentence{Published by Copernicus Publications on behalf of the Arbeitsgemeinschaft Extraterrestrische Forschung e.V.}
  \def\@journalurl{www.astrophys-space-sci-trans.net}
  \def\@journallogo{}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifcp%classical
  \def\@journalname{Climate of the Past}
  \def\@journalnameabbreviation{Clim. Past}
  \def\@journalnameshort{CP}
  \def\@journalnameshortlower{cp}
  \def\@journalstartyear{2005}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.clim-past.net}
    \def\@journallogo{\includegraphics{CP_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.357,0.039,0.475}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.clim-past-discuss.net}
    \def\@journallogo{\includegraphics{CPD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Climate of the Past (CP).\\ Please refer to the corresponding final paper in CP if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.357,0.039,0.475}
      \definecolor{buttonbackground}{rgb}{0.357,0.039,0.475}
      \definecolor{paneltext}{rgb}{0.357,0.039,0.475}
      \definecolor{buttontext}{rgb}{1.0,0.796,0.02}
    \fi
  \fi
\fi
\ifesd%classical
  \def\@journalname{Earth System Dynamics}
  \def\@journalnameabbreviation{Earth Syst. Dynam.}
  \def\@journalnameshort{ESD}
  \def\@journalnameshortlower{esd}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.earth-syst-dynam.net}
    \def\@journallogo{\includegraphics{ESD_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.224,0.455}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.224,0.455}
  \else
    \def\@journalurl{www.earth-syst-dynam-discuss.net}
    \def\@journallogo{\includegraphics{ESDD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Earth System\\ Dynamics (ESD). Please refer to the corresponding final paper in ESD if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.224,0.455}
      \definecolor{buttonbackground}{rgb}{0.0,0.224,0.455}
      \definecolor{paneltext}{rgb}{0.0,0.224,0.455}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifgi%classical
  \def\@journalname{Geoscientific Instrumentation, Methods and Data Systems}
  \def\@journalnameabbreviation{Geosci. Instrum. Method. Data Syst.}
  \def\@journalnameshort{GI}
  \def\@journalnameshortlower{gi}
  \def\@journalstartyear{2012}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geosci-instrum-method-data-syst.net}
    \def\@journallogo{\includegraphics{GI_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.geosci-instrum-method-data-syst-discuss.net}
    \def\@journallogo{\includegraphics{GID_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Geoscientific Instrumentation,\\ Methods and Data Systems (GI). Please refer to the corresponding final paper in GI if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.012,0.306,0.635}
      \definecolor{buttonbackground}{rgb}{0.635,0.635,0.635}
      \definecolor{paneltext}{rgb}{0.012,0.306,0.635}
      \definecolor{buttontext}{rgb}{0.012,0.306,0.635}
    \fi
  \fi
\fi
\ifgmd%classical
  \def\@journalname{Geoscientific Model Development}
  \def\@journalnameabbreviation{Geosci. Model Dev.}
  \def\@journalnameshort{GMD}
  \def\@journalnameshortlower{gmd}
  \def\@journalstartyear{2008}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geosci-model-dev.net}
    \def\@journallogo{\includegraphics{GMD_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.geosci-model-dev-discuss.net}
    \def\@journallogo{\includegraphics{GMDD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Geoscientific Model\\ Development (GMD). Please refer to the corresponding final paper in GMD if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.973,0.584,0.055}
      \definecolor{buttonbackground}{rgb}{0.973,0.584,0.055}
      \definecolor{paneltext}{rgb}{0.973,0.584,0.055}
      \definecolor{buttontext}{rgb}{0.769,0.086,0.11}
    \fi
  \fi
\fi
\ifhess%classical
  \def\@journalname{Hydrology and Earth System Sciences}
  \def\@journalnameabbreviation{Hydrol. Earth Syst. Sci.}
  \def\@journalnameshort{HESS}
  \def\@journalnameshortlower{hess}
  \def\@journalstartyear{1997}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.hydrol-earth-syst-sci.net}
    \def\@journallogo{\includegraphics{HESS_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.hydrol-earth-syst-sci-discuss.net}
    \def\@journallogo{\includegraphics{HESSD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Hydrology and Earth System\\ Sciences (HESS). Please refer to the corresponding final paper in HESS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.38,0.643,0.161}
      \definecolor{buttonbackground}{rgb}{0.38,0.643,0.161}
      \definecolor{paneltext}{rgb}{0.38,0.643,0.161}
      \definecolor{buttontext}{rgb}{0.122,0.153,0.498}
    \fi
  \fi
\fi
\ifnhess%classical
  \def\@journalname{Natural Hazards and Earth System Sciences}
  \def\@journalnameabbreviation{Nat. Hazards Earth Syst. Sci.}
  \def\@journalnameshort{NHESS}
  \def\@journalnameshortlower{nhess}
  \def\@journalstartyear{2001}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.nat-hazards-earth-syst-sci.net}
    \def\@journallogo{\includegraphics{NHESS_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.nat-hazards-earth-syst-sci-discuss.net}
    \def\@journallogo{\includegraphics{NHESSD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Natural Hazards and Earth\\ System Sciences (NHESS). Please refer to the corresponding final paper in NHESS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.263,0.416,0.702}
      \definecolor{buttonbackground}{rgb}{0.69,0.639,0.576}
      \definecolor{paneltext}{rgb}{0.263,0.416,0.702}
      \definecolor{buttontext}{rgb}{0.263,0.416,0.702}
    \fi
  \fi
\fi
\ifnpg%classical
  \def\@journalname{Nonlinear Processes in Geophysics}
  \def\@journalnameabbreviation{Nonlin. Processes Geophys.}
  \def\@journalnameshort{NPG}
  \def\@journalnameshortlower{npg}
  \def\@journalstartyear{1994}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union \& the American Geophysical Union.}
  \if@stage@final
    \def\@journalurl{www.nonlin-processes-geophys.net}
    \def\@journallogo{\includegraphics{NPG_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.nonlin-processes-geophys-discuss.net}
    \def\@journallogo{\includegraphics{NPGD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Nonlinear Processes\\ in Geophysics (NPG). Please refer to the corresponding final paper in NPG if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.102,0.278,0.6}
      \definecolor{buttonbackground}{rgb}{0.996,0.749,0.004}
      \definecolor{paneltext}{rgb}{0.102,0.278,0.6}
      \definecolor{buttontext}{rgb}{0.102,0.278,0.6}
    \fi
  \fi
\fi
\ifos%classical
  \def\@journalname{Ocean Science}
  \def\@journalnameabbreviation{Ocean Sci.}
  \def\@journalnameshort{OS}
  \def\@journalnameshortlower{os}
  \def\@journalstartyear{2005}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.ocean-sci.net}
    \def\@journallogo{\includegraphics{OS_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.ocean-sci-discuss.net}
    \def\@journallogo{\includegraphics{OSD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Ocean Science (OS).\\ Please refer to the corresponding final paper in OS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.039,0.282,0.494}
      \definecolor{buttonbackground}{rgb}{0.039,0.282,0.494}
      \definecolor{paneltext}{rgb}{0.039,0.282,0.494}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifse%classical
  \def\@journalname{Solid Earth}
  \def\@journalnameabbreviation{Solid Earth}
  \def\@journalnameshort{SE}
  \def\@journalnameshortlower{se}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.solid-earth.net}
    \def\@journallogo{\includegraphics{SE_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.solid-earth-discuss.net}
    \def\@journallogo{\includegraphics{SED_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Solid Earth (SE).\\ Please refer to the corresponding final paper in SE if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.482,0.349,0.259}
      \definecolor{buttonbackground}{rgb}{0.482,0.349,0.259}
      \definecolor{paneltext}{rgb}{0.482,0.349,0.259}
      \definecolor{buttontext}{rgb}{0.98,0.922,0.835}
    \fi
  \fi
\fi
\iftc%classical
  \def\@journalname{The Cryosphere}
  \def\@journalnameabbreviation{The Cryosphere}
  \def\@journalnameshort{TC}
  \def\@journalnameshortlower{tc}
  \def\@journalstartyear{2007}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.the-cryosphere.net}
    \def\@journallogo{\includegraphics{TC_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.the-cryosphere-discuss.net}
    \def\@journallogo{\includegraphics{TCD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal The Cryosphere (TC).\\ Please refer to the corresponding final paper in TC if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.341,0.596,0.824}
      \definecolor{buttonbackground}{rgb}{0.341,0.596,0.824}
      \definecolor{paneltext}{rgb}{0.341,0.596,0.824}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifdwes%classical
  \def\@journalname{Drinking Water Engineering and Science Discussions}
  \def\@journalnameabbreviation{Drink. Water Eng. Sci.}
  \def\@journalnameshort{DWES}
  \def\@journalnameshortlower{dwes}
  \def\@journalstartyear{2008}
  \def\@sentence{Published by Copernicus Publications on behalf of the Delft University of Technology.}
  \if@stage@final
    \def\@journalurl{www.drink-water-eng-sci.net}
    \def\@journallogo{\includegraphics{DWES_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.0,0.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{0.0,0.0,0.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.drink-water-eng-sci-discuss.net}
    \def\@journallogo{\includegraphics{DWESD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Drinking Water Engineering and\\ Science (DWES). Please refer to the corresponding final paper in DWES if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.49,0.761}
      \definecolor{buttonbackground}{rgb}{0.0,0.49,0.761}
      \definecolor{paneltext}{rgb}{0.0,0.49,0.761}
      \definecolor{buttontext}{rgb}{0.682,0.824,0.31}
    \fi
  \fi
\fi
\ifessd%classical
  \def\@journalname{Earth System Science Data}
  \def\@journalnameabbreviation{Earth Syst. Sci. Data}
  \def\@journalnameshort{ESSD}
  \def\@journalnameshortlower{essd}
  \def\@journalstartyear{2009}
  \def\@sentence{Published by Copernicus Publications.}
  \if@stage@final
    \def\@journalurl{www.earth-syst-sci-data.net}
    \def\@journallogo{\includegraphics{ESSD_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.102,0.4,0.573}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.earth-syst-sci-data-discuss.net}
    \def\@journallogo{\includegraphics{ESSDD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Earth System Science\\ Data (ESSD). Please refer to the corresponding final paper in ESSD if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.102,0.4,0.573}
      \definecolor{buttonbackground}{rgb}{0.102,0.4,0.573}
      \definecolor{paneltext}{rgb}{0.102,0.4,0.573}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifesurf%classical
  \def\@journalname{Earth Surface Dynamics}
  \def\@journalnameabbreviation{Earth Surf. Dynam.}
  \def\@journalnameshort{ESURF}
  \def\@journalnameshortlower{esurf}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.earth-surf-dynam.net}
    \def\@journallogo{\includegraphics{ESURF_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.541,0.549,0.557}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.earth-surf-dynam-discuss.net}
    \def\@journallogo{\includegraphics{ESURFD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Earth Surface Dynamics (ESurfD).\\ Please refer to the corresponding final paper in ESurf if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.0,0.0}
      \definecolor{buttonbackground}{rgb}{0.541,0.549,0.557}
      \definecolor{paneltext}{rgb}{0.0,0.0,0.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifgh%classical
  \def\@journalname{Geographica Helvetica}
  \def\@journalnameabbreviation{Geogr. Helv.}
  \def\@journalnameshort{GH}
  \def\@journalnameshortlower{gh}
  \def\@journalstartyear{1946}
  \def\@sentence{\small Published by Copernicus Publications for the Geographisch-Ethnographische Gesellschaft Z\"urich \& Association Suisse de G\'eographie.}
  \def\@journalurl{www.geogr-helv.net}
  \def\@journallogo{\includegraphics{GH_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.569,0.58,0.588}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.569,0.58,0.588}
\fi
\ifhgss%classical
  \def\@journalname{History of Geo- and Space Sciences}
  \def\@journalnameabbreviation{Hist. Geo Space Sci.}
  \def\@journalnameshort{HGSS}
  \def\@journalnameshortlower{hgss}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications.}
  \if@stage@final
    \def\@journalurl{www.hist-geo-space-sci.net}
    \def\@journallogo{\includegraphics{HGSS_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.443,0.706}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.443,0.706}
  \else
    \def\@journalurl{https://hgss.copernicus.org/preprints/preprints.html}
    \def\@journallogo{\includegraphics{HGSSD_Logo.pdf}}
    \def\@sentenceDiscussion{This preprint is/has been under review for the journal History of Geo- and Space Sciences (HGSS). Please refer to the corresponding final paper in HGSS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifjsss%classical
  \def\@journalname{Journal of Sensors and Sensor Systems}
  \def\@journalnameabbreviation{J. Sens. Sens. Syst.}
  \def\@journalnameshort{JSSS}
  \def\@journalnameshortlower{jsss}
  \def\@journalstartyear{2012}
  \def\@sentence{Published by Copernicus Publications on behalf of the AMA Association for Sensor Technology.}
  \def\@journalurl{www.j-sens-sens-syst.net}
  \def\@journallogo{\includegraphics{JSSS_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.051,0.298,0.561}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.051,0.298,0.561}
\fi
\ifms%classical
  \def\@journalname{Mechanical Sciences}
  \def\@journalnameabbreviation{Mech. Sci.}
  \def\@journalnameshort{MS}
  \def\@journalnameshortlower{ms}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications.}
  \def\@journalurl{www.mech-sci.net}
  \def\@journallogo{\includegraphics{MS_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.471,0.655,0.808}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{0.0,0.0,0.0}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifasr%classical
  \def\@journalname{Advances in Science and Research}
  \def\@journalnameabbreviation{Adv. Sci. Res.}
  \def\@journalnameshort{ASR}
  \def\@journalnameshortlower{asr}
  \def\@journalstartyear{2007}
  \def\@sentence{Published by Copernicus Publications.}
  \def\@journalurl{www.adv-sci-res.net}
  \def\@journallogo{\includegraphics{ASR_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.004,0.302,0.545}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.004,0.302,0.545}
\fi
\ifsdsr%classical
  \def\@journalname{Scientific Drilling - Science Reports}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.075,0.239,0.553}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.075,0.239,0.553}
\fi
\ifsdpr%classical
  \def\@journalname{Scientific Drilling - Progress Reports}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.906,0.651,0.278}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.906,0.651,0.278}
\fi
\ifsdtd%classical
  \def\@journalname{Scientific Drilling - Technical Developments}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.722,0.094,0.141}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{0.722,0.094,0.141}
\fi
\ifsdwr%classical
  \def\@journalname{Scientific Drilling - Workshop Reports}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.486,0.298,0.216}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.486,0.298,0.216}
\fi
\ifsdpd%classical
  \def\@journalname{Scientific Drilling - Program Developments}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.027,0.498,0.325}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.027,0.498,0.325}
\fi
\ifwe%classical
  \def\@journalname{Web Ecology}
  \def\@journalnameabbreviation{Web Ecol.}
  \def\@journalnameshort{WE}
  \def\@journalnameshortlower{we}
  \def\@journalstartyear{2001}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Ecological Federation (EEF).}
  \def\@journalurl{www.web-ecol.net}
  \def\@journallogo{\includegraphics{WE_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.2,0.6,0.2}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.2,0.6,0.2}
\fi
\ifangeocom%classical
  \def\@journalname{AnGeo Communicates}
  \def\@journalnameabbreviation{Ann. Geophys.}
  \def\@journalnameshort{ANGEOCOM}
  \def\@journalnameshortlower{angeo}
  \def\@journalstartyear{1983}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.ann-geophys.net}
    \def\@journallogo{\includegraphics{ANGEO_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{0.851,0.851,0.851}
    \definecolor{rulecol}{rgb}{0.0,0.0,0.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifsoil%classical
  \def\@journalname{SOIL}
  \def\@journalnameabbreviation{SOIL}
  \def\@journalnameshort{SOIL}
  \def\@journalnameshortlower{soil}
  \def\@journalstartyear{2015}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.soil-journal.net}
    \def\@journallogo{\includegraphics{SOIL_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.29,0.267,0.165}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.29,0.267,0.165}
  \else
    \def\@journalurl{www.soil-discuss.net}
    \def\@journallogo{\includegraphics{SOILD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal SOIL. Please refer to the\\ corresponding final paper in SOIL if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.29,0.267,0.165}
      \definecolor{buttonbackground}{rgb}{0.29,0.267,0.165}
      \definecolor{paneltext}{rgb}{0.29,0.267,0.165}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifpb%classical
  \def\@journalname{Primate Biology}
  \def\@journalnameabbreviation{Primate Biol.}
  \def\@journalnameshort{PB}
  \def\@journalnameshortlower{pb}
  \def\@journalstartyear{2014}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsches Primatenzentrum GmbH (DPZ).}
  \def\@journalurl{www.primate-biol.net}
  \def\@journallogo{\includegraphics{PB_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.0,0.0,0.0}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{0.0,0.0,0.0}
\fi
\ifascmo%classical
  \def\@journalname{Advances in Statistical Climatology, Meteorology and Oceanography}
  \def\@journalnameabbreviation{Adv. Stat. Clim. Meteorol. Oceanogr.}
  \def\@journalnameshort{ASCMO}
  \def\@journalnameshortlower{ascmo}
  \def\@journalstartyear{2015}
  \def\@sentence{Published by Copernicus Publications.}
  \def\@journalurl{www.adv-stat-clim-meteorol-oceanogr.net}
  \def\@journallogo{\includegraphics{ASCMO_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.392,0.039,0.039}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.392,0.039,0.039}
\fi
\ifpiahs%classical
  \def\@journalname{Proceedings of the International Association of Hydrological Sciences}
  \def\@journalnameabbreviation{Proc. IAHS}
  \def\@journalnameshort{PIAHS}
  \def\@journalnameshortlower{piahs}
  \def\@journalstartyear{1924}
  \def\@sentence{Published by Copernicus Publications on behalf of the International Association of Hydrological Sciences.}
  \def\@journalurl{proc-iahs.net}
  \def\@journallogo{\includegraphics{PIAHS_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.553,0.035,0.035}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.553,0.035,0.035}
\fi
\ifaab%classical
  \def\@journalname{Archives Animal Breeding}
  \def\@journalnameabbreviation{Arch. Anim. Breed.}
  \def\@journalnameshort{AAB}
  \def\@journalnameshortlower{aab}
  \def\@journalstartyear{2015}
  \def\@sentence{Published by Copernicus Publications on behalf of the Research Institute for Farm Animal Biology (FBN).}
  \def\@journalurl{www.arch-anim-breed.net}
  \def\@journallogo{\includegraphics{AAB_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.6,0.0,0.0}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifwes%classical
  \def\@journalname{Wind Energy Science}
  \def\@journalnameabbreviation{Wind Energ. Sci.}
  \def\@journalnameshort{WES}
  \def\@journalnameshortlower{wes}
  \def\@journalstartyear{2016}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Academy of Wind Energy e.V.}
  \if@stage@final
    \def\@journalurl{www.wind-energ-sci.net}
    \def\@journallogo{\includegraphics{WES_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.075,0.263,0.565}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.075,0.263,0.565}
  \else
    \def\@journalurl{www.wind-energ-sci-discuss.net}
    \def\@journallogo{\includegraphics{WESD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Wind Energy Science (WES).\\ Please refer to the corresponding final paper in WES if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.075,0.263,0.565}
      \definecolor{buttonbackground}{rgb}{0.075,0.263,0.565}
      \definecolor{paneltext}{rgb}{0.075,0.263,0.565}
      \definecolor{buttontext}{rgb}{0.584,0.761,0.239}
    \fi
  \fi
\fi
\ifjm%classical
  \def\@journalname{Journal of Micropalaeontology}
  \def\@journalnameabbreviation{J. Micropalaeontology}
  \def\@journalnameshort{JM}
  \def\@journalnameshortlower{jm}
  \def\@journalstartyear{1982}
  \def\@sentence{Published by Copernicus Publications on behalf of The Micropalaeontological Society.}
  \def\@journalurl{www.j-micropalaeontol.net/}
  \def\@journallogo{\includegraphics{JM_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.047,0.306,0.427}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{0.047,0.306,0.427}
\fi
\ifegqsj%classical
  \def\@journalname{E&G Quaternary Science Journal}
  \def\@journalnameabbreviation{E\&G Quaternary Sci. J.}
  \def\@journalnameshort{EGQSJ}
  \def\@journalnameshortlower{egqsj}
  \def\@journalstartyear{1951}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsche Quart\"arvereinigung (DEUQUA) e.V.}
  \def\@journalurl{www.eg-quaternary-sci-j.net}
  \def\@journallogo{\includegraphics{EGQSJ_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.0,0.459,0.722}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifgc%classical
  \def\@journalname{Geoscience Communication}
  \def\@journalnameabbreviation{Geosci. Commun.}
  \def\@journalnameshort{GC}
  \def\@journalnameshortlower{gc}
  \def\@journalstartyear{2018}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geosci-commun.net}
    \def\@journallogo{\includegraphics{GC_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.067,0.494,1.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{0.067,0.494,1.0}
  \else
    \def\@journalurl{www.geosci-commun-discuss.net}
    \def\@journallogo{\includegraphics{GCD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifdeuquasp%classical
  \def\@journalname{DEUQUA Special Publications}
  \def\@journalnameabbreviation{DEUQUA Spec. Pub.}
  \def\@journalnameshort{DEUQUASP}
  \def\@journalnameshortlower{deuquasp}
  \def\@journalstartyear{2018}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsche Quart\"arvereinigung (DEUQUA) e.V.}
  \def\@journalurl{www.deuqua-spec-pub.net}
  \def\@journallogo{\includegraphics{DEUQUASP_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.529,0.533,0.541}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifgchron%classical
  \def\@journalname{Geochronology}
  \def\@journalnameabbreviation{Geochronology}
  \def\@journalnameshort{GCHRON}
  \def\@journalnameshortlower{gchron}
  \def\@journalstartyear{2019}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geochronology.net}
    \def\@journallogo{\includegraphics{GCHRON_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.447,0.247,0.329}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.geochronology-discuss.net}
    \def\@journallogo{\includegraphics{GCHROND_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Geochronology (GChron).\\ Please refer to the corresponding final paper in GChron if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifwcd%classical
  \def\@journalname{Weather and Climate Dynamics}
  \def\@journalnameabbreviation{Weather Clim. Dynam.}
  \def\@journalnameshort{WCD}
  \def\@journalnameshortlower{wcd}
  \def\@journalstartyear{2019}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.weather-clim-dynam.net}
    \def\@journallogo{\includegraphics{WCD_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.weather-clim-dynam-discuss.net}
    \def\@journallogo{\includegraphics{WCDD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifejm%classical
  \def\@journalname{European Journal of Mineralogy}
  \def\@journalnameabbreviation{Eur. J. Mineral.}
  \def\@journalnameshort{EJM}
  \def\@journalnameshortlower{ejm}
  \def\@journalstartyear{1989}
  \def\@sentence{Published by Copernicus Publications on behalf of the European mineralogical societies DMG, SEM, SIMP \& SFMC.}
  \def\@journalurl{www.eur-j-mineral.net}
  \def\@journallogo{\includegraphics{EJM_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.0,0.0,0.0}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifmr%classical
  \def\@journalname{Magnetic Resonance}
  \def\@journalnameabbreviation{Magn. Reson.}
  \def\@journalnameshort{MR}
  \def\@journalnameshortlower{mr}
  \def\@journalstartyear{2020}
  \def\@sentence{Published by Copernicus Publications on behalf of the Groupement AMPERE.}
  \if@stage@final
    \def\@journalurl{www.magn-reson.net}
    \def\@journallogo{\includegraphics{MR_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.627,0.098,0.086}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{\includegraphics{MRD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifjbji%classical
  \def\@journalname{Journal of Bone and Joint Infection}
  \def\@journalnameabbreviation{J. Bone Joint Infect.}
  \def\@journalnameshort{JBJI}
  \def\@journalnameshortlower{jbji}
  \def\@journalstartyear{2016}
  \def\@sentence{Published by Copernicus Publications on behalf of EBJIS and MSIS.}
  \def\@journalurl{https://jbji.copernicus.org/}
  \def\@journallogo{\includegraphics{JBJI_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.161,0.337,0.361}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.161,0.337,0.361}
\fi
\ifpolf%classical
  \def\@journalname{Polarforschung - Journal of the German Society for Polar Research}
  \def\@journalnameabbreviation{Polarforschung}
  \def\@journalnameshort{POLF}
  \def\@journalnameshortlower{polf}
  \def\@journalstartyear{1931}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsche Gesellschaft für Polarforschung e.V.}
  \def\@journalurl{https://polf.copernicus.org}
  \def\@journallogo{\includegraphics{POLF_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.306,0.525,0.682}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifsand%classical
  \def\@journalname{Safety of Nuclear Waste Disposal}
  \def\@journalnameabbreviation{Saf. Nucl. Waste Disposal}
  \def\@journalnameshort{SAND}
  \def\@journalnameshortlower{sand}
  \def\@journalstartyear{2021}
  \def\@sentence{Published by Copernicus Publications on behalf of the Federal Office for the Safety of Nuclear Waste Management (BASE).}
  \def\@journalurl{www.sand.copernicus.org}
  \def\@journallogo{\includegraphics{SAND_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.0,0.0,0.0}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.0,0.0,0.0}
\fi
\ifegusphere%classical
  \def\@journalname{EGUsphere}
  \def\@journalnameabbreviation{EGUsphere}
  \def\@journalnameshort{EGUSPHERE}
  \def\@journalnameshortlower{egusphere}
  \def\@journalstartyear{2022}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{https://egusphere.copernicus.org}
    \def\@journallogo{\includegraphics{EGUSPHERE_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{https://egusphere.copernicus.org}
    \def\@journallogo{\includegraphics{EGUSPHERE_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.0,0.0}
      \definecolor{buttonbackground}{rgb}{0.0,0.0,0.0}
      \definecolor{paneltext}{rgb}{0.0,0.0,0.0}
      \definecolor{buttontext}{rgb}{0.0,0.0,0.0}
    \fi
  \fi
\fi

}
